Chern-Simons bubbles: Lopsided false vacuum decay in axion electrodynamics

We study axion electrodynamics, including the Chern-Simons interaction term, in the presence of parallel background electric and magnetic fields, as can for example occur in certain models of axion inflation and in the study of dyonic black holes. In this setup, we find a new back-reacted instanton solution which corresponds to the nucleation of an axion domain wall that screens the electromagnetic fields in a process analogous to Schwinger pair production, despite the absence of light charged particles. The full solution includes the effect of the Chern-Simons induced charges and currents on the axion domain wall arising from the Witten and Sikivie (anomalous Hall) effects, respectively. The Euclidean solution has a reduced $O(2)\times O(2)$ symmetry which describes the nucleation of a prolate bubble in its rest-frame. A unique feature of this solution is that the region of lower energy density is outside the bubble rather than inside. We also describe the time evolution of this initial configuration, showing how the bubble can become further elongated along the direction of the background electric and magnetic fields. We describe potential applications of this process in particle physics and cosmology.

==> preamble.tex <==
%\documentclass[11pt,letterpaper]{article}
%\pdfoutput=1
\usepackage{jheppub}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{subfig}
\usepackage{bbold}
\usepackage{tabularx}
\usepackage[makeroom]{cancel}
\usepackage{multirow}
\usepackage{slashed}
\usepackage{hyperref}


\newcommand{\Mpl}{M_\mathrm{Pl}}
\newcommand{\Mbh}{M_\mathrm{BH}}
\newcommand{\Mgut}{M_\mathrm{GUT}}





\title{False vacuum decay in axion electrodynamics}


\author{Saquib Hassan,}
\author{John March-Russell,}
\author{and Georges Obied}


\emailAdd{saquib.hassan@physics.ox.ac.uk} 
\emailAdd{john.march-russell@physics.ox.ac.uk}
\emailAdd{georges.obied@physics.ox.ac.uk}

\affiliation{Rudolf Peierls Centre for Theoretical Physics \\University of Oxford \\OX1 3PU Parks Road \\ Oxford \\ United Kingdom}

\date{\today}

\bibliographystyle{JHEP}
